Dynamic interactions between an aerodynamic flow and a flexible flat plate

Passive flow control via fluid-structure interaction (FSI) is a promising paradigm for unmanned aerial vehicles operating in vortex-dominated low Reynolds number regimes. A flexible structure has the potential to passively alter key unsteady vortex structures through its vibrations if its intrinsic modal dynamics are carefully aligned with the driving flow processes. Towards this aim, we perform high-fidelity numerical FSI simulations to study the dynamic interplay between a separated aerodynamic flow with vortex shedding (Re = 500 and angle of attack of 15$^{\circ}$) and a flexible flat plate modeled using linear Euler-Bernoulli beam theory. To isolate the natural evolution/instability mechanisms of the coupled dynamics, we start our simulations from a steady base state of the FSI system. We focus on open questions related to the coupled dynamics: (i) Do the early-time dynamics that evolve from the base state involve a coupled or flow-driven instability?; (ii) how are the flow dynamics and associated lift informed by the modal shape(s) and deformation timescales of the structural response, and how is this structural response informed by the structural parameters relative to the vortex-shedding behavior of the reference (rigid) case? For question (i), we identify that the departure from the base state arises from a flow-induced instability, suggesting that it is the vortex shedding of the aerodynamic flow that instigates structural motion. For question (ii), we further clarify how the structural mode dynamics in the FSI setting are dictated by the relationship between the vacuum fundamental frequencies of the structure and the baseline rigid-plate shedding frequency. We show that the long-time FSI dynamics can be partitioned into distinct regimes categorized by the dominant mode of the structural dynamics. The coupled dynamics in each regime are described in detail in the manuscript.

==> figures/overviewfigures_1/meancl.tex <==
\begin{tikzpicture}[]
\begin{loglogaxis}[%
enlargelimits=false, 
axis on top, 
%axis equal image, 
width=7cm,
xlabel=$m$,
ylabel=$\overline{Cl}$,
%xticklabels={,,},
%yticklabels={0.5,1},
tick align=inside,
]
\addplot graphics [xmin=0.0001,xmax=100,ymin=0.8329,ymax=1.0533]{figures/overviewfigures_1/meancl.png};



\end{loglogaxis}



\end{tikzpicture}


==> figures/overviewfigures_1/midptextrema.tex <==
\begin{tikzpicture}[]
\begin{semilogxaxis}[%
enlargelimits=false, 
axis on top, 
%axis equal image, 
width=7cm,
xlabel=$m$,
ylabel=$\chi_{mid}$,
%xticklabels={,,},
%yticklabels={0.5,1},
tick align=inside,
]
\addplot graphics [xmin=0.0001,xmax=100,ymin=-0.1,ymax=0.15]{figures/overviewfigures_1/midptpoincare.png};



\end{semilogxaxis}



\end{tikzpicture}

